From Pixels to Tokens: A Systematic Study of Latent Action Supervision for Vision-Language-Action Models

Latent actions serve as an intermediate representation that enables consistent modeling of vision-language-action (VLA) models across heterogeneous datasets. However, approaches to supervising VLAs with latent actions are fragmented and lack a systematic comparison. This work structures the study of latent action supervision from two perspectives: (i) regularizing the trajectory via image-based latent actions, and (ii) unifying the target space with action-based latent actions. Under a unified VLA baseline, we instantiate and compare four representative integration strategies. Our results reveal a formulation-task correspondence: image-based latent actions benefit long-horizon reasoning and scene-level generalization, whereas action-based latent actions excel at complex motor coordination. Furthermore, we find that directly supervising the VLM with discrete latent action tokens yields the most effective performance. Finally, our experiments offer initial insights into the benefits of latent action supervision in mixed-data, suggesting a promising direction for VLA training. Code is available at https://github.com/RUCKBReasoning/From_Pixels_to_Tokens.

==> sections/method_0110.tex <==
Latent actions are introduced as a form of training-time supervision, without modifying the inference-time architecture or computational cost.
Following the two classes of latent actions defined in Section~3.2, four hypotheses are formulated to study how latent actions influence policy learning, as shown in Figure~\ref{fig:figure2}. Hypotheses~1--3 focus on image-based latent actions and are presented in Section~4.1, while Hypothesis~4 considers action-based latent actions and is described together with its instantiation in Section~4.2. For image-based latent actions, an existing pretrained latent action model is adopted (details provided in Appendix~\ref{app_details_image}.). 

\subsection{Image-based Latent Actions for VLA}
\label{section4.1}
\subsubsection{Hypothesis 1: Representation Alignment}
We hypothesize that image-based latent actions can serve as a high-level semantic regularizer, encouraging intermediate action-token representations to align with visually grounded visual-transition semantics.
This hypothesis relies on the assumption that there exists a relatively low-entropy mapping from visual transitions to action semantics, it may fail in settings where such embeddings are highly multimodal or weakly aligned with actionable control features.

From a representation learning perspective, intermediate layers of VLMs tend to encode shared and task-agnostic semantics, while later layers increasingly specialize toward low-level continuous control through the action head~\cite{wang2025vla}.
Based on this assumption, we impose a representation-level consistency constraint that encourages intermediate action-token hidden states to align with the embedding space induced by image-based latent actions, and apply this constraint at an intermediate VLM layer.

Formally, let $h_t \in \mathbb{R}^d$ denote the hidden representation of the $t$-th action token extracted from an intermediate VLM layer.
Since the two representations may reside in different feature spaces, we introduce a lightweight projection function $\phi(\cdot)$ to map action-token representations into the latent-action embedding space.
The representation alignment objective is defined as
\begin{equation}
\mathcal{L}_{\mathrm{align}}
= - \mathbb{E}_{t}
\Big[
\mathcal{S}\big( \phi(h_t),\, z_t^{\mathrm{img}} \big)
\Big],
\end{equation}
where $\mathcal{S}(\cdot,\cdot)$ is used to compute alignment, and we employ cosine similarity for this purpose.
The latent action model is kept fixed during training, and gradients are propagated only through the VLA backbone and the projection function $\phi$.

The overall training objective augments the standard action prediction loss with the alignment regularizer:
\begin{equation}
\mathcal{L}
= \mathcal{L}_{\mathrm{action}} + \lambda_{\mathrm{align}} \mathcal{L}_{\mathrm{align}},
\end{equation}
where $\lambda_{\mathrm{align}}$ controls the strength of the regularization.

\subsubsection{Hypothesis 2: Discrete Latent Action Supervision}

We hypothesize that discrete latent actions learned from short-horizon visual transitions constitute a compact, low-entropy abstraction of action-relevant dynamics, and can therefore serve as structured and stable supervision for action prediction. By decoupling high-level transition semantics from low-level control, latent actions enable a hierarchical formulation of the action policy.

Formally, given an observation $o_t$ and a language instruction $\ell$, the action policy is factorized through a discrete latent action variable $c_t$:
\begin{equation}
\pi(a_t \mid o_t, \ell)
= \sum_{c_t} \pi_\phi(a_t \mid c_t^{\mathrm{img}}, s_t)\, \pi_\theta(c_t^{\mathrm{img}} \mid o_t, \ell),
\end{equation}
As defined previously, $c_t^{\mathrm{img}}$ is a discrete code that captures essential action-induced dynamics while discarding low-level nuisance variations.

During training, we align the latent action inferred from inputs $(o_t, \ell)$ with the discrete latent action extracted from visual transitions, and use it as supervision for VLM. Specifically, the latent action inference model is trained using cross-entropy loss:
\begin{equation}
\label{latent_loss}
\mathcal{L}_{\mathrm{latent}}
= \mathbb{E}_{t}\left[ - \log \pi_\theta(c_t^{\mathrm{img}} \mid o_t, \ell) \right].
\end{equation}

The final training objective combines latent action supervision with continuous action prediction:
\begin{equation}
\mathcal{L}
= \mathcal{L}_{\mathrm{action}}
+ \lambda_{\mathrm{latent}}\, \mathcal{L}_{\mathrm{latent}},
\label{eq:latent}
\end{equation}
where $\lambda_{\mathrm{latent}}$ controls the relative strength of latent supervision. Importantly, latent action supervision is applied only during training; the inference-time architecture and computational cost remain unchanged.

\subsubsection{Hypothesis 3: Coarse-to-Fine Action Decoding}

We hypothesize that placing latent action tokens as a prefix within the action decoding segment can induce a coarse-to-fine organization of action generation. The key difference from Hypothesis~2 is the internal dependency structure encouraged by the placeholder composition: latent tokens are decoded first to provide a high-level motion context, and low-level continuous actions are decoded subsequently conditioned on this latent prefix.

Concretely, for each time step $t$, we consider a single action-decoding segment that contains (i) a latent-token prefix and (ii) an action-token suffix. Denoting the discrete latent action code by $c_t$ and the continuous action representation by $\hat{a}_t$, Hypothesis~3 encourages the following coarse-to-fine factorization:
\begin{equation}
\begin{aligned}
\pi(\hat{a}_t, c_t \mid o_t, \ell)
&=
\prod_{k=1}^{K}
\pi_\theta\!\left(
c_{t,k} \mid o_t, \ell, c_{t,<k}
\right) \\
&\quad \times
\prod_{m=1}^{M}
\pi_\phi\!\left(
a_{t,m} \mid o_t, \ell, c_t, a_{t,<m}
\right).
\end{aligned}
\end{equation}

Latent prefix is trained with cross-entropy objective,
\begin{equation}
\mathcal{L}_{\mathrm{latent}}
=
\mathbb{E}_{t}\left[
- \sum_{j=1}^{L} \log \pi_\theta(c_{t,j}^{\mathrm{img}} \mid o_t, \ell, c_{t,<j}^{\mathrm{img}})
\right],
\label{eq:h3_vlm_latent_only_token}
\end{equation}
The overall objective remains as Eq.~\ref{eq:latent}.

Importantly, this hypothesis changes how the model \emph{organizes} action decoding by injecting a latent-token prefix into the same action placeholder segment, thereby biasing the decoder toward a coarse-to-fine organization. We do not claim that latent tokens are human-interpretable rationales; rather, they function as compact internal variables that shape the organization of low-level action decoding.

\subsection{Action-based Latent Actions}
\label{section4.2}
\subsubsection{Hypothesis 4: Action-to-Token Mapping}
\label{sec:hypothesis4}

Action-based latent actions embed continuous control signals into the language model token space. By mapping actions to discrete tokens that share the same embedding space as language, this design enables pretrained language representations to directly interact with and reason over action semantics.

Unlike Hypothesis~2, here latent actions are obtained directly from continuous actions. We assume access to a fixed, pretrained action-based latent action model, which deterministically maps each continuous action $a_t \in \mathbb{R}^m$ to a discrete latent code, each discrete code $c_t^{\mathrm{act}}$ corresponds to a learned codebook embedding $g(c_t^{\mathrm{act}}) \in \mathbb{R}^d$, where $d$ matches the dimensionality of the language model token embeddings.
As a result, action-induced semantics are represented as discrete tokens that reside in the same embedding space as natural language tokens.

From a modeling perspective, Hypothesis~4 adopts the same latent-variable formulation as Hypothesis~2.
Specifically, given an observation $o_t$ and a language instruction $\ell$, the action policy is factorized through the discrete latent action variable $c_t^{\mathrm{act}}$:
\begin{equation}
\pi(a_t \mid o_t, \ell)
= \sum_{c_t^{\mathrm{act}}} \pi_\phi(a_t \mid c_t^{\mathrm{act}}, s_t)\, \pi_\theta(c_t^{\mathrm{act}} \mid o_t, \ell),
\end{equation}
where the latent action $c_t^{\mathrm{act}}$ is now obtained from an action-based encoder.

During post-training, action placeholders in the language model are supervised to predict the corresponding action-based latent tokens.
Following Hypothesis~2, the latent action inference model is trained using a token-level cross-entropy objective (Eq.~\ref{latent_loss}).
The overall training objective remains identical to Eq.~\ref{eq:latent}.

\subsubsection{Instantiating Action-based Latent Actions}

\begin{figure}[!ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.6\columnwidth]{Figures/Figure_3.pdf}}
\caption{Architecture of the action-based latent action model.}
\label{fig:figure3}
\end{center}
\vskip -0.2in
\end{figure}

To instantiate Hypothesis~4, we adopt an action-based latent action model that directly tokenizes short sequences of continuous actions into a temporally aligned sequence of discrete latent tokens.
Given a fixed-length action chunk $\mathbf{a}_{1:T} = (a_1,\ldots,a_T)$ with $a_t \in \mathcal{A} \subset \mathbb{R}^m$, the model produces a corresponding latent action token sequence
$\mathbf{k}_{1:T} = (k_1,\ldots,k_T)$, where each $k_t \in \{1,\ldots,K\}$ indexes a learned codebook entry.

Concretely, the model first encodes the action sequence into a sequence of continuous latent representations using a temporal encoder that combines local convolutional structure with global self-attention:
\begin{equation}
\mathbf{u}_{1:T} = E_{\psi}(\mathbf{a}_{1:T}), \qquad \mathbf{u}_{1:T} \in \mathbb{R}^{T \times d}.
\end{equation}
Each latent representation is then discretized via vector quantization: $k_t = \mathrm{VQ}(\mathbf{u}_t), \qquad k_t \in \{1,\ldots,K\}$, 
and decoded back to the action space through a lightweight decoder: $\hat{a}_t = D_{\psi}\!\left(g(k_t)\right)$.

The model is trained to shape the semantics of latent action tokens using a combination of reconstruction and consistency objectives.
First, an action reconstruction loss ensures that the discrete tokens preserve sufficient information to recover the underlying control signals:
\begin{equation}
\mathcal{L}_{\mathrm{rec}}
= \mathbb{E}\!\left[
\left\| \mathbf{a}_{1:T} - \hat{\mathbf{a}}_{1:T} \right\|_2^2
\right].
\end{equation}
Second, to encourage temporal coherence and capture local regularities in the latent token sequence, we impose a masked latent consistency objective that predicts masked latent representations from their unmasked context:
\begin{equation}
\mathcal{L}_{\mathrm{mask}}
= \mathbb{E}\!\left[
\left\| E_{\psi}(\hat{\mathbf{a}}_{1:T})_t - \mathbf{u}_t \right\|_2^2
\right],
\end{equation}
where the expectation is taken over masked time steps.

The final training objective additionally includes the standard vector-quantization commitment loss,
\begin{equation}
\mathcal{L}_{\mathrm{ALA}}
=
\mathcal{L}_{\mathrm{rec}}
+ \lambda_{\mathrm{mask}}\,\mathcal{L}_{\mathrm{mask}}
+ \lambda_{\mathrm{vq}}\,\mathcal{L}_{\mathrm{vq}},
\end{equation}
where $\mathcal{L}_{\mathrm{vq}}$ denotes the standard vector-quantization
commitment and codebook loss as in VQ-VAE~\cite{van2017neural},
and $\lambda_{\mathrm{mask}}$ and $\lambda_{\mathrm{vq}}$ balance reconstruction fidelity, temporal consistency, and codebook utilization.

After training, the model defines a fixed, deterministic tokenization from continuous actions to discrete latent indices. These latent action tokens are subsequently used as supervision targets (Section~\ref{sec:hypothesis4}).

% \begin{algorithm}[t]
% \caption{Action-based Latent Action Tokenizer Training}
% \label{alg:action_tokenizer}
% \begin{algorithmic}[1]
% \STATE \textbf{Input:} action chunk $\mathbf{a}_{1:T} \in \mathbb{R}^{T \times m}$; encoder $E_\psi$; vector quantizer $\mathrm{VQ}$ with codebook size $K$; decoder $D_\psi$; mask ratio $\rho$; loss weights $\lambda_{\mathrm{mask}}, \lambda_{\mathrm{vq}}$
% \STATE \textbf{Output:} trained encoder $E_\psi$, codebook, and decoder $D_\psi$
% \FOR{each training step}
%     \STATE \textbf{Time--Frequency Augmentation}
%     \STATE Compute frequency-domain features $\mathcal{F}(\mathbf{a}_{1:T})$ using DCT or FFT
%     \STATE $\tilde{\mathbf{a}}_{1:T} \leftarrow [\mathbf{a}_{1:T}, \mathcal{F}(\mathbf{a}_{1:T})]$
    
%     \STATE \textbf{Temporal Encoding}
%     \STATE $\mathbf{u}_{1:T} \leftarrow E_\psi(\tilde{\mathbf{a}}_{1:T}), \quad \mathbf{u}_{1:T} \in \mathbb{R}^{T \times d}$
    
%     \STATE \textbf{Latent Masking}
%     \STATE Sample mask set $\mathcal{M} \subset \{1,\ldots,T\}$ with ratio $\rho$
%     \STATE Set $\mathbf{u}_t \leftarrow 0$ for all $t \in \mathcal{M}$
    
%     \STATE \textbf{Vector Quantization}
%     \STATE $k_t \leftarrow \mathrm{VQ}(\mathbf{u}_t), \quad k_t \in \{1,\ldots,K\}$
%     \STATE $\mathbf{z}_t \leftarrow g(k_t)$
    
%     \STATE \textbf{Decoding}
%     \STATE $\hat{\mathbf{a}}_{1:T} \leftarrow D_\psi(\mathbf{z}_{1:T})$
    
%     \STATE \textbf{Loss Computation}
%     \STATE $\mathcal{L}_{\mathrm{rec}} \leftarrow \|\mathbf{a}_{1:T} - \hat{\mathbf{a}}_{1:T}\|_2^2$
%     \STATE $\mathcal{L}_{\mathrm{mask}} \leftarrow \|E_\psi(\hat{\mathbf{a}}_{1:T})_t - \mathbf{u}_t\|_2^2 \;\; \forall t \in \mathcal{M}$
%     \STATE $\mathcal{L} \leftarrow \mathcal{L}_{\mathrm{rec}} + \lambda_{\mathrm{mask}}\mathcal{L}_{\mathrm{mask}} + \lambda_{\mathrm{vq}}\mathcal{L}_{\mathrm{vq}}$
    
%     \STATE \textbf{Parameter Update}
%     \STATE Update $E_\psi$, $D_\psi$, and the codebook parameters using gradient descent on $\mathcal{L}$
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}
